A High-Throughput FPGA Accelerator for Lightweight CNNs With Balanced Dataflow

FPGA accelerators for lightweight neural convolutional networks (LWCNNs) have recently attracted significant attention. Most existing LWCNN accelerators focus on single-Computing-Engine (CE) architecture with local optimization. However, these designs typically suffer from high on-chip/off-chip memory overhead and low computational efficiency due to their layer-by-layer dataflow and unified resource mapping mechanisms. To tackle these issues, a novel multi-CE-based accelerator with balanced dataflow is proposed to efficiently accelerate LWCNN through memory-oriented and computing-oriented optimizations. Firstly, a streaming architecture with hybrid CEs is designed to minimize off-chip memory access while maintaining a low cost of on-chip buffer size. Secondly, a balanced dataflow strategy is introduced for streaming architectures to enhance computational efficiency by improving efficient resource mapping and mitigating data congestion. Furthermore, a resource-aware memory and parallelism allocation methodology is proposed, based on a performance model, to achieve better performance and scalability. The proposed accelerator is evaluated on Xilinx ZC706 platform using MobileNetV2 and ShuffleNetV2.Implementation results demonstrate that the proposed accelerator can save up to 68.3% of on-chip memory size with reduced off-chip memory access compared to the reference design. It achieves an impressive performance of up to 2092.4 FPS and a state-of-the-art MAC efficiency of up to 94.58%, while maintaining a high DSP utilization of 95%, thus significantly outperforming current LWCNN accelerators.

==> chapters/sentence.tex <==
These fixed dataflow designs result in a sub-optimal on-chip buffer size and off-chip memory access when running different layers of a CNN with different characteristics.

Nevertheless, the lack of an in-hardware flexible data reuse and shortcut reuse reduces the MAC efficiency. Whereas, the proposed hardware/software co-optimizer, while being fast, provides adaptive data reuses to minimize the off-chip memory access and improve the MAC efficiency even with the on-chip buffer constraints.




==> chapters/tmp/Experiments_v1.tex <==
\section{Experiments}
% 之后，面向ZC706板卡，以ShuffleNetV2和MobileNetV2为目标网络，最小化SRAM和满足FPGA片上BRAM约束的版本被分别实现并与理论性能进行了比较。
% 
This experiment section first describes evaluation results about memory occupation and computing efficiency based on the performance model.
With ShuffleNetV2 and MobileNetV2 as the target networks and Xilinx ZC706 board as the target deployment platform, 
four accelerator versions which minimize the SRAM size and satisfy the BRAM constraints of the target FPGA are then implemented respectively.
Finally, we compare the proposed acceleraor with state-of-the-art LWCNN-oriented accelerators.
% \subsection{Experimental Setup}
\subsection{Simulation Results}
To evaluate the effectiveness and generality of the proposed architecture,
four representative LWCNNs, 
including ShuffleNetV2 ($\times$0.5)\cite{ma2018shufflenet}, ShuffleNetV1\cite{zhang2018shufflenet}, ShuffleNetV2\cite{ma2018shufflenet}, MobileNetV2\cite{sandler2018mobilenetv2}, MobileNetV1\cite{howard2017mobilenets}, MobileNetV2 ($\times$1.4)\cite{sandler2018mobilenetv2},
are taken as the benchmarks for memory and computing simulation.
The main structure of these models are built by extensively stacking DSCs and SCBs.
% Table \ref{tab:eva_net} lists the size and complexity comparisons of these LWCNN models.
For all the above LWCNNs, with 224 $\times$ 224 input image size, they are quantized to 8-bit precision for both weights and activations.
% to enable higher efficiency.
% 量化精度损失低于xxx
% 评估过程基于前面提出的算法完成。在评估完成后，以ZC706为目标板卡，我们部署了SF2和MB2以进一步验证所提出的方案。
% 设计语言为sv，综合与实现通过xilinx vivado2021.2
% 受限于片上资源， 我们根据经验选择存储资源和计算资源的峰值为xxx以实现最好的tradeoff,DSP被拆分以xxxx
% 

% 6个不同规模的网络被选择
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}

% \begin{table}[]
% \renewcommand{\arraystretch}{1.1}
% \caption{Different Lightweight CNNs for Performance Evaluation}
% \label{tab:eva_net}
% \resizebox{\linewidth}{!}{%
% \begin{threeparttable}
% \begin{tabular}{|c|c|c|c|c|}
% \hline
% Network Models      & Params & MACs & Layers\tnote{2} & Top-1 err\tnote{3} \\ \hline
% ShuffleNetV1\tnote{1}        & 1.9M   & 143M & 50       & 33.6\%    \\ \hline
% ShuffleNetV2        & 2.3M   & 146M & 57     & 30.6\%    \\ \hline
% MobileNetV1         & 4.2M   & 569M & 28     & 29.4\%    \\ \hline
% MobileNetV2         & 3.4M   & 300M & 53     & 28.0\%    \\ \hline
% \end{tabular}%
% \begin{tablenotes}    
%         \footnotesize    
%         \item[1] ShuffleNetV1 (group = 1)
%         \item[2] Only computing layers (STC, PWC, DWC and FC) are included 
%         \item[3] The Top-1 classification error for ImageNet dataset.       
%       \end{tablenotes}   
% \end{threeparttable}
% }
% \end{table}

% 仅统计计算层，包括DWC，PWC，DWC和FC
% 评估算法遍历了所有层以寻找满足SRAM约束情况下的最小DRAM访问量，
% 由于特征图复用层具有权重部署片上的特性，
% 在浅层部署特征图复用层时，由于节约了大量特征图存储空间，对SRAM和DRAM占用均存在正面收益。当到达权重较大的深层时，特征图存储优化的收益开始小于权重存储的负面影响，导致SRAM开始增加。
% 随着特征图复用层数量的增加，，
% 对于Mb2最小的sram分界层在xxx，对应sram size是xxx, 而shf由于较小的size,最小sram占用量仅需0.7M，而对于具有2000个bram的目标板卡，在满足BRAM要求下，cut point可以被进一步推进，此时片外访存量降低到xx和xxx。
\begin{figure*}[!t]
    \centering
    \subfloat[]{\includegraphics[width=0.47\linewidth]{blaeva_mb2.png}\label{fig:blaeva_mb2}} ~~~~ \quad
    \subfloat[]{\includegraphics[width=0.47\linewidth]{blaeva_sf2.png}\label{fig:blaeva_sf2}}%
     \caption{Low computational density operations in LWCNNs. (a) Depthwise Separable Convolution(DSC). (b) Skip-Connection Block(SCB).}
    \label{fig:mem eva}
\end{figure*}

Based on the memory allocation algorithm in Section.~\ref{sec:mem alloc}.
Fig.~\ref{fig:mem eva} illustrates  the SRAM size and DRAM access of our hybrid CE architecture with respect to the boundary location for ShuffleNetV2 and MobileNetV2.
The evaluation algorithm sequentially searches through all layers to find the minimum DRAM access that satisfies the SRAM constraints.
deploying shallow layers with FRCE favors for both SRAM and DRAM utilization due to the massive reuse for middle activation.
% When deploying shallow layers with FRCE, there are significant benefits for both SRAM and DRAM utilization due to the massive reuse for middle activation.
As the convert layer reaches the deeper layers with larger weights, 
the contribution brought by the line buffer could not counteract the negative impact of the weight ROM, which aggravate the SRAM consumption.
% the contribution brought by line buffers is smaller than the negative impact of weight ROM, which aggravate the SRAM consumption.
The minimum SRAM required for MobileNetV2 is 1.27MB corresponding to layer conv12-2,
while 0.71 MB SRAM is sufficient for ShuffleNetV2 due to its small model size.
For the target FPGA with 545 BRAMs, the group boundary can be further advanced until reaching the BRAM constraints, where the off-chip access can be reduced from 2.81MB and 1.96MB to 2.05 MB and 0.98 MB, respectively.
In the subsequent discussions, the accelerator with minimum SRAM size will be used as the default version for performance comparison.
% 后续讨论中默认使用最小SRAM版本作为性能比较依据。

\begin{figure}[!t]
\centerline{\includegraphics[width=\linewidth]{figure/ram cmp3.png}}
    \caption{Architecture of the proposed accelerator.}
    \label{fig:sram cmp}
\end{figure}

% 在这两种方案中，只有全连接层的数据由于低权重复用率被存储在片外
% For fully connected layers, the weights are stored in DRAM due to their lower reuse rate。

% 在浅层中，相比于行复用方案，Linebuffer size 与scb size的使用被有效减少。比如，在同样权重存储方案的情况下，full reuse bixxx 特征图缓存减少了xxx。
% 与行复用方案相比，特征图全局复用方案可以有效减少Linebuffer size 与scb size的使用，由于最大程度的减少了数据的生命周期，在同样权重存储方案的情况下，采用特征图全局复用模式的specific方案相比于baseline将Linebuffer缓存和scb缓存平均减少了116.0%和150.1%。
% 在深层中，由于采用了单一的复用方案，现有方案很容易导致大量用于权重数据的sram消耗。相比之下，得益于混合的数复用方案，本方案将权重存储减少了xxx，即使全局特征图存储导致了额外的全局数据缓存，在消耗少量DRAM访存为代价的情况下，sram占用量仍然比现有方案降低了约一倍。
% 用来提取高纬度信息
% 这一特点在shufflenet中相反
% We can see that the size of line buffer is bigger than SCB buffer in MobileNetV2.

Fig.~\ref{fig:sram cmp} presents the on-chip buffer size comparison of the proposed design over other streaming architectures, where "baseline" means processing LWCNNs with the line-based weight reuse strategy, while "specific" represents using the FM fully reused strategy for all convolution layers to minimize local FM size.
Note that the weights of FC layers in evaluated schemes are not included for a reasonable comparison.
% Note that the weights of FC layers in evaluated schemes are stored in DRAM for a reasonable comparison.
The size of the line buffer is observed to be larger than the SCB buffer in MobileNetV2. 
this is because the inverted residual block for high-dimension information extraction has higher number of input channels in the middle layers than the SCB entrance.
This feature is reversed in ShuffleNetV1 for similar reason.
Benefit from the higher FM reuse rate, the size requirement for Line buffer and SCB buffer in specific scheme is reduced by 116.0\% and 150.1\% , respectively,  compared with the baseline scheme, demonstrating that the reduction for data life cycle leads a positive effect for the FM buffer size in streaming accelerators.
As for deep layers, the existing scheme can easily incur a large amount of SRAM consumption for weight data due to their fixed data reuse scheme. 
In contrast, 
the weight storage of the proposed accelerator with hybrid data reuse scheme are 436.8\% lower on average than that of comparison schemes. 
Even though the fully reused weight requires additional GFM buffer, 
the overall SRAM footprint is still approximately  half the size of existing schemes at the cost of a small amount of DRAM access.
\begin{figure}[!t]
\centerline{\includegraphics[width=\linewidth]{figure/dram cmp.png}}
    \caption{Architecture of the proposed accelerator.}
    \label{fig:dram cmp}
\end{figure}
% Benefit from the reduced data ife cycle, the size requirement for Line buffer and scb buffer 
% 在单次前向过程中，由于数据在CE间的传输消耗，层间和SCB中的FM访存均被有效移除。
% 权重数据访存也得到部分减少,达到xx  
% 在xx网络中最多减少xxxx
% 对于访存需求更大的LWCNN，我们的多CE架构在某种程度进一步拓展了SE架构，使得几乎所有特征图数据都可以在CE间传输，从而避免了频繁的数据交换，
% 此外，混合的复用与存储策略也相应减少了权重的访问次数与访问量。
% repetitive exchange of activations between external memories and on-chip memories
% 为了便于展示，Shortcut数据被单独统计出来以更好的展示对SCB结构的访存优化 
% 在MobilenetV2中，与UE结构相比，FM访存，SCB访存和权重访存分别减少了5%,10%,20%，

Fig.~\ref{fig:dram cmp} exhibits the off-chip memory traffic comparison among UE, SE and the proposed architectures during each inference of the LWCNN procesing,
where shortcut data is presented separately from FM data for better illustration.
Without loss of validity, we assume that all data in UE architecture are accessed off-chip exactly once, while the SE architecture 
further eliminate the FM access for DWC layers. 
For LWCNNs with heavy FM access requirements, our streaming architecture further extends the SE architecture so that all middle FM data can be transferred among CEs, thus avoiding frequent exchange of activations between external memories and on-chip memories.
Out of this, the hybrid reuse and storage strategy correspondingly reduces the bandwidth requirement for weights in terms of both access times and data quantity.
As a result, the proposed architecture requires only 2.95MB for DRAM access during MobileNetV2 processing, 
resulting in a 95.2\%, 16.5\% and 98.9\% reduction for Shortcut data, Weights and FMs, respectively.
% Compared to the UE architecture,  reduces the total DRAM access by 253.8\%-492.2\% for the various LWCNNs.
% \begin{figure}[!t]
%     \centering
%     % \subfloat[]{\includegraphics[width=0.5\linewidth]{mb1cmp.png}\label{fig:blaeva_mb2}} ~~~~ \quad
%     \subfloat[]{\includegraphics[width=0.45\linewidth]{figure/effcmp.png}}\label{fig:blaeva_sf2}
%     \subfloat[]{\includegraphics[width=0.45\linewidth]{effcmp.png}\label{fig:blaeva_sf2}}
%      \caption{Low computational density operations in LWCNNs. (a) Depthwise Separable Convolution(DSC). (b) Skip-Connection Block(SCB).}
%     \label{fig:lwcnn operation}
% \end{figure}
\begin{figure*}[!t]
    \centering
    % \subfloat[]{\includegraphics[width=0.5\linewidth]{mb1cmp.png}\label{fig:blaeva_mb2}} ~~~~ \quad
    \subfloat[]{\includegraphics[width=0.5\linewidth]{mb2cmp.png}\label{fig:blaeva_sf2}}
    % \subfloat[]{\includegraphics[width=0.5\linewidth]{sf1cmp.png}\label{fig:blaeva_sf2}} ~~~~ \quad
    \subfloat[]{\includegraphics[width=0.5\linewidth]{sf2cmp.png}\label{fig:blaeva_sf2}}%
     \caption{Low computational density operations in LWCNNs. (a) Depthwise Separable Convolution(DSC). (b) Skip-Connection Block(SCB).}
    \label{fig:lwcnn operation}
\end{figure*}

\begin{figure}[!t]
\centerline{\includegraphics[width=\linewidth]{figure/effcmp.png}}
    \caption{Architecture of the proposed accelerator.}
    \label{fig:effcmp}
\end{figure}
% \begin{figure}[!t]
% \centerline{\includegraphics[width=\linewidth]{figure/dram cmp.png}}
%     \caption{Architecture of the proposed accelerator.}
%     \label{fig:mix mem}
% \end{figure}



% 1.平均效率提升，相同的设计约束
% 2.可拓展性好，即，数据波动小
% 3.常规方式的不足，在sf2中更加明显
% 为了论证FGPM在多CE系统的有效性，我们也基于动态并行度调整算法评估了在相同的设计约束下FGPM相比传统方案的理论吞吐率和可拓展性方面的提升，其中Mb2和sf2的评估过程如图所示。
% 的在，其中baseline指的是使用因子并行粒度进行并行度切分，我们在相同的设计约束下通过动态并行度调整算法依次增加MAC的数量
% 我们可以看出传统方案的吞吐率变化有着明显的阶梯效应，这是由于增加的计算资源无法被用于有效提升瓶颈层的吞吐率。
% 这一现象在大多数通道都难以分解的shufflentv2中更加明显，
% 相比之下，本方案的吞吐率随着MAC数量的增加有着近乎线性的变化关系，表明在大多数场景中增加的计算资源有效的参与了计算，从而取得了更高的计算效率。
% 我们总结了四个网络从60到4000个MAC的评估过程中的平均计算效率和标准差以更好的说明，其中标准差数据通过衡量系统的性能变化的稳反映系统的可拓展性定程度反映系统的可拓展性
% 其中标准差数据通过衡量加速器在不同MAC数量下的性能的离散程度反映系统的可拓展性
% 相比于基准方案,本方案在Shufflenet V2中取了了高达31.29%的计算性能提升，这因为shuf2v2的大部分通道数量设置难以分解出充足的整数因子，因此FGPM增加了并行空间并因此对整体性能有利
% 基于FGPM的不同MAC数量下的平均理论MAC效率可以达到93-95%，相比于基准方案提升了10%-32%。
% 除了计算效率，FGPM在4个网络中的标准差数据也取得了明显优势，证明了该方案在计算资源方面具有更好的泛化性能。
%  in Fig. 3 for better clarity.
To demonstrate the effectiveness of FGPM in multi-CE systems,
We also evaluate the enhancement in terms of theoretical throughput and scalability of FGPM compared to baseline schemes which commonly employed in many streaming accelerators with the same design constraints.
The evaluation process for MobileNetV2 and ShuffleNetV2 driven by Dynamic Parallelism Tuning algorithm is shown in Fig.~\ref{fig:lwcnn operation}.
We can see that the throughput of the baseline scheme has a significant step effect, which is caused by the fact that the increased computing resources remain underutilized and thus have no contribution to the throughput of the bottleneck layers. 
This problem is even worse in ShuffleNetv2 since most channels are difficult to decompose and generate sufficient integer factors.
In contrast, the throughput of our scheme has a nearly linear relationship as the growth of MACs, indicating that the increased computing resources effectively participate in the computation in most cases and thus achieving a higher computing efficiency.
We unify the average efficiency and standard deviation from 60 to 4000 MACs in Fig.~\ref{fig:effcmp} for better illustration, where the standard deviation reflects the generalization performance by measuring the dispersion of the accelerator's performance with different numbers of MACs.
The average theoretical MAC efficiency based on FGPM with different number of MACs can achieve 93.06-95.68\% for four benchmark networks, which is a 6.46-32.19\% improvement compared to the baseline.
furthermore, the reduction in standard deviation also demonstrate that our scheme has a better scalability for platforms with diverse computing resources.
% FGPM also achieves a significant advantage in the standard deviation, demonstrating that our scheme has better generalization performance.
% Compared to the baseline scheme, our scheme achieves up to 31.29\% computing performance improvement in ShuffleNetV2.
% This is because most of the channel number in ShuffleNetV2 are hard to decompose to provide sufficient parallel levels, and thus FGPM increases the parallelism space and thus favors the overall performance.
% by  measuring the degree of dispersion of the accelerator performance with .  
% by measuring the stability of the accelerator's performance variation.
%by  measuring the degree of dispersion of the accelerator performance variation.  


\subsection{Implementation Results}
% DWC中计算密度太低，少量增加的计算资源也无法被充分消化，这也部分说明了为什么绝大多数加速器处理DSC的效率很低。
% 1.图能不能充实一点    2.如何展示padding opt
% part1  results, comparison with ideal,mem and computing

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
 \renewcommand{\arraystretch}{1.1}
\caption{Resource Utilization}
\label{tab:resource}
\resizebox{\linewidth}{!}{%
\begin{tabular}{|c|c|c|c|c|}
\hline
             & LUT             & DFF             & BRAM36K        & DSP          \\ \hline
Available    & 218600          & 437200          & 545            & 900          \\ \hline
MobileNetV2  & 163087 (74.61\%) & 189476 (43.34\%) & 329.5 (60.46\%) & 844 (93.78\%) \\ \hline
ShuffleNetV2 & 117554 (53.78\%) & 177863 (40.68\%) & 209 (38.35\%)   & 853 (94.78\%) \\ \hline
\end{tabular}%
}
\end{table}
To further validate the proposed methodologies, we implement the MobileNetV2 and ShuffleNetV2 accelerators on a Xilinx ZC706 board according to the evaluated Mini SRAM version in Fig.~\ref{fig:mem eva}, respectively.
As for computing resources, we empirically adopt the maximum DSP utilization at 95\% (855 DSPs) for the Dynamic Parallelism Tuning algorithm to achieve the best trade-off between timing performance and resource utilization.
the DSP decomposition is also deployed in our accelerator by performing two 8 $\times$ 8 multipliers in one DSP48E1 to increase the peak performance except in DWC layer with independent channels.
As a result, our accelerators run at frequency of 200MHZ and the resource utilization is listed in Table \ref{tab:resource}.
% we decompose each DSP48E1 into two 8 $\times$ 8 multipliers with one input sharing the same value to increase the overall performance. This method is not deployed in DWC CE since each channel is independent in DWC.
% part2 performance enhancement

% part3 
\subsection{Related Works}






% Unlike the traditional single-CE accelerators, which are
% difficult to achieve linear performance improvement or are not
% scalable, the proposed accelerator maintains high computational efficiency while improving fine-grained throughput by
% allocating a small amount of computational resources to the
% bottleneck layers.





















% % 6个不同规模的网络被选择
% % Please add the following required packages to your document preamble:
% % \usepackage{graphicx}
% \begin{table}[]
% \renewcommand{\arraystretch}{1.1}
% \caption{Different Lightweight CNNs for Performance Evaluation}
% \label{tab:eva_net}
% \resizebox{\linewidth}{!}{%
% \begin{threeparttable}
% \begin{tabular}{|c|c|c|c|c|}
% \hline
% Network Models      & Params & MACs & Layers\tnote{2} & Top-1 err\tnote{3} \\ \hline
% ShuffleNetV2 ($\times$0.5) & 1.4M   & 41M  & 57     & 39.7\%    \\ \hline
% ShuffleNetV1\tnote{1}        & 1.9M   & 143M & 50       & 33.6\%    \\ \hline
% ShuffleNetV2        & 2.3M   & 146M & 57     & 30.6\%    \\ \hline
% MobileNetV2         & 3.4M   & 300M & 53     & 28.0\%    \\ \hline
% MobileNetV1         & 4.2M   & 569M & 28     & 29.4\%    \\ \hline
% MobileNetV2 ($\times$1.4)  & 6.9M   & 585M & 53     & 25.3\%    \\ \hline
% \end{tabular}%
% \begin{tablenotes}    
%         \footnotesize    
%         \item[1] ShuffleNetV1 (group = 1)
%         \item[2] Only computing layers (STC, PWC, DWC and FC) are included 
%         \item[3] The Top-1 classification error for ImageNet dataset.       
%       \end{tablenotes}   
% \end{threeparttable}
% }
% \end{table}
% % 仅统计计算层，包括DWC，PWC，DWC和FC

==> chapters/tmp/intro.tex <==
\section{Introduction}
\IEEEPARstart{I}{n} recent years, convolutional neural networks (CNNs) have achieved remarkable success in computer vision applications such as image classification\cite{krizhevsky2017imagenet, tripathy2022convolutional, simonyan2014very}, object detection\cite{redmon2016you, zaidi2022survey}, and semantic segmentation\cite{rethink21,salama2021deep, malhotra2022deep}. 
% The current mainstream trend in the development of CNNs is to improve their accuracy by augmenting their size and depth. 
% Enhancing CNN's size and depth is the current mainstream trend to increase model's accuracy. 
% However, the high computational complexity leads to an increase in the required computing and storage resources for deployment, which poses many challenges for the application of CNNs.
% However, CNN models' high computational complexity leads to a consequent increase in the computational and storage resources required for deployment.
% However, the high computational complexity of CNN models increases the amount of computational and storage resources required for deployment.
However, a large number of operations and parameters in typical CNNs require high computational and storage overhead to realize real-time inference,
which makes it difficult to deploy on edge and embedded devices with power and resource restrictions.
To reduce the model size, various model compression techniques, e.g., pruning\cite{jacob2018quantization, toward20, EdgeSide24} and lower-bit quantization\cite{wang2018design, nagel2021white}, have been introduced.
Additionally, lightweight convolutional neural networks (LWCNNs), such as MobileNet\cite{howard2017mobilenets,sandler2018mobilenetv2} and ShuffleNet\cite{zhang2018shufflenet,ma2018shufflenet}, have also been proposed with significantly reduced model complexity and acceptable accuracy. 
Nevertheless,
their efficiency on general computing platforms such as CPU and GPU is still relatively low\cite{yu2020light}.
Therefore, tremendous research attention is focused on FPGA-based dedicated LWCNN accelerators.
% Therefore, increasing research attention is focused on FPGA-based dedicated LWCNN accelerators.

% Consequently, a lot of attention has been given to LWCNN by both academics and industry.
% % By adopting a more efficient and compact structure, lightweight neural networks can eliminate a large number of parameters and computations, making them more suitable for deployment in resource-constrained scenarios.
% % Lightweight neural network can reduce many parameters and computations by using a more effective and compact structure, which makes them better suited for deployment in resource-constrained scenarios.
% LWCNNs are more suitable for deployment in resource-constrained scenarios as they can decrease numerous parameters and calculations by employing a more efficient and compact structure.
% Nevertheless,The efficiency of LWCNNs on general computing platforms such as CPU and GPU is still unsatisfactory in high-speed applications\cite{watanabe2014architectures} with high frame rate requirements or energy-efficient edge devices\cite{yu2020light}, such as self-driving automobiles, high-speed robotics, and drones. 
% Therefore, it is crucial to design specific hardware accelerator architecture for LWCNNs.

\begin{figure}[!t]
\centerline{\includegraphics[width=\linewidth]{struc percentage.png}}
    \caption{Percentage of DSC and SCB structures in major LWCNNs.}
    \label{fig:percentage}
\end{figure}
% Among LWCNNs, DSC\cite{howard2017mobilenets} and BLO structure\cite{xie2019fast} are essential in model structure to minimize model size with acceptable performance.
% % standard convolution(STC) is divided into deepwise convolution(DWC) and point convolution(PWC) in DSC. 
% The two components of DSC—deepwise convolution(DWC) and point convolution(PWC)—replace the original computation-intensive STC.
% PWC is standard convolution with a kernel size of 1$\times$1, while DWC extracts only local information from feature map on each channel, resulting in shrink of computations and parameters.
% % PWC is standard convolution with a kernel size of 1x1, while DWC extract only local information from feature map on each channel resulting in shrink for number of parameters and calculations. 
% % The BLO structure, which consists of multiple 1$\times$1 and 3$\times$3 convolutional layers, is derived from residual module in ResNet\cite{he2016deep}, which uses shortcut connections to address the vanishing gradients during deep neural networks training.
% The BLO structure, which uses shortcut connections to address the vanishing gradients during deep neural networks training and consists of multiple 1$\times$1 and 3$\times$3 convolutional layers, is derived from residual module in ResNet\cite{he2016deep}.
% The combination of BLO structure and DSC in networks such as ShuffleNetV2, MobileNetV2, etc. has achieved excellent results in terms of network size and accuracy.
% Table 1 displays the usage of DSC and BLO in lightweight neural networks. 
% The BLO makes up 60\%–70\% of the model's total number of layers, while the DSC makes up 70\%–80\% of the model.
% A significant percentage of the model's structure and computational complexity is accounted for by DSC and BLO,
% demonstrating that the computational optimization of the DSC and BLO is key to the design of the accelerator.

Depthwise separable convolutions (DSCs) and skip-connection blocks (SCBs) play an essential role in realizing compact and efficient LWCNN models.
DSC decomposes a standard convolution (STC) into a depthwise convolution (DWC) followed by a pointwise convolution (PWC),  
which greatly reduces the amount of computation and parameters.
SCBs, derived from ResNet\cite{he2016deep}, utilize short connections to mitigate the accuracy degradation problem during the training of deep networks.
As shown in Fig.~\ref{fig:percentage}, DSCs and SCBs account for a significant percentage of model structure, and thus optimizing these components is key for accelerator design.
However, 
both structures reduce data reuse opportunities and operational intensity, 
leading to high requirements for data bandwidth and low computational efficiency in LWCNN implementation.
% resulting in a significant shrink of both computations and parameters.

\IEEEpubidadjcol
% 他们中的大部分聚焦于具有局部优化的单CE架构，一些工作改变PE架构使ce可以同时支持DWC和STC，一些工作为DWC设计特定的计算引擎从而减少中间数据流，对于SCB结构xxx结构被提出。
% 仅支持单一的数据复用方案，导致次优的片外访存或片上空间。
% 此外，LWCNN增大了各层中计算量、访存量和层结构差异，单一CE中固定的计算资源映射和数据复用方式难以精准满足各层对计算量和访存量的需求，因此导致了较低的计算效率。
% 此外，LWCNN 中各层特征图形状、权重大小、计算方式和计算量差异较大，将所有计算资源映射到单个或两个计算引擎的资源映射方式较为单一，也会影响计算效率，难以实现所有层的高效运行。
To support LWCNNs efficiently, a number of hardware accelerators have been introduced. 
Most of them focus on single-Computing-Engine (CE) architectures with local optimization to decrease data communication or improve PE efficiency.
References \cite{bai2018cnn,yu2020light} slice and map DWC into a unified convolution CE so that the DWC layers can get a higher computational parallelism.  
To reduce intermediate FM transfers, a dedicated CE is deployed to conduct DWC layer separately\cite{wu2019high,wu2021flexible,knapheide2020high}.
By this means, the operations in DWC and PWC layers can be paralleled in a pipeline mode with a lower latency.
In contrast, \cite{xie2019fast} makes use of partial fusion dataflow to relieve the bandwidth burden of SCB,
while \cite{yan2021fpga} employs an extra input buffer for SCB input to eliminate the data transmission between on-chip and off-chip memory.  
However, all of these works essentially execute LWCNNs with a single CE and a fixed data reuse scheme.  
Their layer-by-layer dataflow demands either heavy off-chip memory traffic produced by frequent FM and weight accesses or large on-chip buffer footprint\cite{DepFiN23}, which degrades system efficiency.
Meanwhile, the common computational resource mapping and fixed data reuse scheme in a single CE may not fit well for the bandwidth or computing resource requirement of each layer \cite{maximizing17, highutilization22, yolotiny24} since LWCNN enlarges the differences between layers in terms of data shape and the number of operations. 
This generally leads to lower computational efficiency (less than 50\%) and accordingly produces a significant gap between the actual and theoretical throughput. 
Furthermore, most of the above works still face the problem of insufficient utilization of computing resources. 
Their DSP utilization on deployed FPGA is normally less than 70\%, and they are not scalable, which results in unnecessary performance loss.
% Their layer-by-layer dataflow requires either heavy off-chip memory traffic produced by frequent FM and weight accesses or large on-chip buffer footprint.
% Meanwhile, the fixed computational resource mapping and common data reuse scheme in a single CE may not fit well for the computation or access requirement of each layer \cite{yolotiny24, highutilization22} since LWCNN enlarges the differences between layers in terms of data shape and the number of operations.
% This inevitably leads to lower computational efficiency, typically less than 50\%. 
% Meanwhile, LWCNN enlarges the differences between layers in terms of data shape and the number of operations, making it difficult for the fixed computational resource mapping and common data reuse scheme in a single CE to meet the computation and access requirement of each layer. 

% 基于LWCNN中特征图和权重大小具有固定的分布趋势，我们提出了一种方案
% 相比于采用固定计算资源映射方案的加速器，MAC efficiency最高提升了5.8倍
To address these issues,
a streaming-based architecture with hybrid CEs is first proposed to relieve considerable FM bandwidth stress caused by DSCs and SCBs.
On the observation of local data dependency between contiguous layers and the distributions of FM and weight size in LWCNN,
our accelerator fully reuses the intermediate results between CEs to minimize DRAM access for middle FMs,
while Feature map Reused CE (FRCE) and Weight Reused CE (WRCE) are deployed for shallow layers and deep layers, respectively, to decrease on-chip memory overhead as well as weight access.
The on-chip memory occupation is reduced by 56.7\% relative to the state-of-the-art streaming accelerator for LWCNN in \cite{jiang2023high} with modest off-chip traffic and the same target model.
Then, a balanced dataflow strategy is designed to improve the computing efficiency of our multi-CE-based accelerator from two perspectives, namely,
fine-grained parallel mechanism to enlarge parallel space and thus enable efficient resource mapping at a theoretical level, 
while dataflow-oriented buffer optimization can relieve data congestion at an implementation level.
Up to 5.8$\times$ MAC efficiency improvement is achieved compared to previous single-CE-based architecture with a common computing resource mapping scheme\cite{yan2021fpga}.
Furthermore,
Since DSP utilization and CE type can be flexibly adjusted based on highly parameterized CE design,  
A resource allocation methodology is proposed to explore the design space and leverage the limited computing and memory resources on the target platform.
We evaluate the proposed architecture with four representative LWCNNs and further implement our accelerator on ShuffleNetV2 and MobileNetV2 in accordance with the above techniques. A high performance of 2092.4 FPS and an almost full load MAC efficiency of 94.58\% are achieved, which outperforms the previous works.
% Compared to the state-of-the-art, our work achieves 5.3× DSP efficiency and 5.5× energy efficiency.

% A resource allocation methodology is proposed to improve the scalability of our architecture and leverage the limited computing and memory resources on the target platform.

The main contributions of this paper are given as follows:
\begin{itemize}
% \item We propose a streaming-based architecture with hybrid CEs to maximize intermediate FM reuse of LWCNNs while decreasing on-chip memory overhead. 
\item A streaming-based architecture with hybrid CEs is proposed to minimize on-chip memory overhead as well as off-chip access, where the FRCE targets optimizing the size of FM buffer for shallow layers while the WRCE aims at maximizing off-chip weight reuse for deep layers.
\item A balanced dataflow strategy including a fine-grained parallel mechanism and dataflow-oriented buffer optimization is proposed to enhance the computing efficiency through efficient resource mapping and data congestion mitigation, respectively. 
\item Based on a performance model, A resource-aware memory and parallelism allocation methodology is proposed to improve the scalability of our accelerator so that the accelerator can make full use of available resources to further enhance system performance.
\end{itemize}


% \item Based on a performance model, A resource-aware memory and parallelism allocation methodology is proposed to improve the scalability of our architecture so that our accelerator can make full use of available resources to further enhance system performance.
The rest of this paper is organized as follows. 
Section II introduces the background and motivation. 
Section III proposes the accelerator with hybrid CEs. 
In Section IV, a balanced dataflow strategy is introduced based on our architecture. 
Section V discusses the resource allocation algorithm. 
Section VI shows the experimental results.
Finally, the conclusion is drawn in Section VII.







 

==> chapters/tmp/line_buffer_scheme.tex <==
\subsection{Dataflow-oriented Padding scheme}
\begin{figure}[!t]
    \centering
    \centerline{\includegraphics[width=\linewidth]{legend for conges.png}}
    % \subfig{\includegraphics[width=\linewidth]{legend for conges.png}}
    \subfloat[]{\includegraphics[width=0.45\linewidth]{paddinga.png}\label{fig:paddinga}} ~~
    \subfloat[]{\includegraphics[width=0.45\linewidth]{paddingb.png}\label{fig:paddingb}}\\
    \subfloat[]{\includegraphics[width=0.45\linewidth]{paddingc.png}\label{fig:paddingc}} ~~
    \subfloat[]{\includegraphics[width=0.45\linewidth]{paddingd.png}\label{fig:paddingd}}\\
    % \subfloat{\includegraphics[width=\linewidth]{legend for conges.png}\label{fig:shufflenetv2fmw}}
     \caption{Memory requirements for FMs and Weights in LWCNNs. The data for each block is the sum of all the layers within it (a) MobileNetV2. (b) ShuffleNetV2.}
    \label{fig:padding}
\end{figure}

\begin{figure}[!t]
    \centering
    \subfloat[]{\includegraphics[width=0.45\linewidth]{s2a.png}\label{fig:paddinga}} ~~
    \subfloat[]{\includegraphics[width=0.45\linewidth]{s2b.png}\label{fig:paddingb}}
    % \subfloat{\includegraphics[width=\linewidth]{legend for conges.png}\label{fig:shufflenetv2fmw}}
     \caption{Memory requirements for FMs and Weights in LWCNNs. The data for each block is the sum of all the layers within it (a) MobileNetV2. (b) ShuffleNetV2.}
    \label{fig:s2}
\end{figure}
% 低效的padding操作
% padding:缓存空间不匹配
% 当输入的特征图大小与输出大小不
% 为了保证输入输出特征图大小相同采用padding操作增加了需要处理的数据量，方案xx采用将padding数据写入line buffer的缓存方式，不但
Another crucial issue affecting the computational efficiency of streaming architectures is data congestion, which is mainly caused by inefficient padding implementation.
The padding operation is a process of supplementing zeros at the edge of the FM to prevent information loss.
these zero values break the original FM data sequence and increase total data amount, posing challenge on contiguous bandwidth supplement for the PE array.
% This poses a challenge on limited block ram bandwidth and generally requires extra complicated data reuse management (like line buffer) to accomplish.

% 其次，有着较低信息密度的padding值会占据用于上层输入数据存储的位置，压缩了弹性缓存空间
% 假设卷积核大小为$3 \times 3$，在特征图的四周进行padding。
% 在直接插入方式中，写入的padding数据可以和普通像素一样用于前一张图片的运算。但是，由于缓存空间减少，在当上一张特征图的卷积完成时，需要在Row buffer中额外缓存一行输入特征图才能开始卷积的计算
Existing works \cite{RealTimeObject18, yan2021fpga, LowPowerMobil23} normally insert zeros directly into the input FMs before feeding them into the line buffer,
and then perform convolution operation with padding data function as general pixels.
This comes with two issues, i.e.data backpressure for the preceding CE and invalid convolution windows in the current CE.
On the one hand,
Writing the padding value to the Row buffer will take up the write bandwidth of the Row buffer, which results in either a large input buffer to store input pixels or a computing stall in the preceding CE. 
Furthermore, 
Padding values with lower information density occupy precious memory space for input pixel, incurring invalid convolution windows during image switching process.
Fig.~\ref{fig:padding}\subref{fig:paddinga} and Fig.~\ref{fig:padding}\subref{fig:paddingb} depicts the direct insertion approach in convolution layer with $3 \times 3$ kernel size and same padding pattern, 
where the padding data is reused and processed in both the last row of the previous image and the first row of the next.
After generating the last window of the previous FM, 
an additional row of input pixels is required to be cached in the Line buffer to form the first active window of next FM.
which inevitably leads to interrupted data supply and the idle state of PE.
% padding data functions as normal pixels during the adjacent image computation process,
% 在这相邻的两张图像处理过程中，填充数据与正常像素采用相同的方式存储和计算，
% padding数据即参与前一张图片的最后一行，又参与后一张图像第一行的运算
% the padding data can be used as normal pixels for both the computation of the last image
% 在这种场景
% Interrupted data supply is caused in this scenario, which low hardware utilization overhead, the idle state of the CE 


% In this work, a Dataflow-oriented Padding scheme is proposed to increase hardware computing efficiency via promising sufficient bandwidth supply.
% Considering the uniformity of padding data and its specific insertion locations,
% the padding operation is performed by address controller while the pixels are sending to PE array instead of being written into the line buffer as input pixels,
% which avoid congestion of upstream data.
% More importantly, 
% the padding data generated by the address logic indirectly increases the input bandwidth and thus effectively removes window bubbles when switching images.
% As shown in Fig.~\ref{fig:padding}\subref{fig:paddingc} and Fig.~\ref{fig:padding}\subref{fig:paddingd},
% Since the occupation of row buffer by padding data is avoided, 
% a new line of pixels have been stored in the line buffer when the previous image is completed, 
% Combined with the supplemented padding data,
% the subsequent FM can start a new round of convolutional computation without any delay, which greatly reduce the hardware resource idle.

In this work, a Dataflow-oriented Padding scheme is proposed to increase hardware computing efficiency via promising sufficient bandwidth supply.
Considering the uniformity of padding data and its specific insertion locations,
the padding operation is performed by the address controller while the pixels are sending to PE array instead of being written into the line buffer as input pixels,
which avoids the congestion of upstream data.
More importantly, 
the padding data generated by the address logic indirectly increases the input bandwidth and thus effectively removes window bubbles when switching images.
As shown in Fig.~\ref{fig:padding}\subref{fig:paddingc} and Fig.~\ref{fig:padding}\subref{fig:paddingd},
Since the occupation of row buffer by padding data is avoided, 
a new line of pixels have been stored in the line buffer when the previous image is completed, 
Combined with the supplemented padding data,
the subsequent FM can start a new round of convolutional computation without any delay, which greatly reduce the hardware resource idle.
For convolution layers with stride = 2, 
an extra line buffer is allocated in our scheme to eliminate window bubbles caused by a mismatch between limited buffer space and required data scope. 
with extra buffer space and an efficient padding generator, 
the computing efficiency of DWC layers with a diverse range of padding locations and strides can be effectively improved.
% our padding scheme  the computational efficiency at different .
% 此外，对步长大于一的深度卷积层，典型值为2.我们的Padding方案会分配额外的行Buffer，用来消除因卷积步长较大导致的窗口气泡，不同的buffer个数结合逻辑控制的padding生成器，可以有效保证在不同步长和不同padding方案的计算效率。
% 此外，部分深度卷积层步长大于一，典型值为2.额外的行Buffer会被我们的Padding方案分配用来消除因有限的缓存空间和更大的数据局部性不匹配而导致的窗口气泡，不同的buffer个数结合逻辑控制的padding生成器，可以有效保证在不同步长和不同padding方案的计算效率。


% 我们的方案在特征图较小的层具有更显著的优化效果，以图的内容为例进行量化分析，对于F大小的特征图，假设输入数据持续不断写入Row buffer，
% 如果采用上述传统padding方案使用的时间约为$(F+2)(F+1) \times Speed_{write}$，而本文提出的流驱动padding生成器消耗的时间为$F^2 \times Speed_{write}$。
% 加速效果$Radio_{acc}$可以用式\ref{equ:padding radio}进行评估。在加速Mobilenet v2网络时，单层最高可以取得约1.6倍的带宽提升。
% 我们的方案可以有效减少padding的特征图缓存时间，对于特征图较小的层性能提升更高
% The Dataflow-oriented Padding scheme can achieve higher performance improvement for layers with smaller feature maps. 
% 对于padding数据占总特征图比例越大的层，我们的方案优化效果越明显
% 对单层来说，我们的方案的加速效率和padding数据占输入特征图比例成正相关，
% With our Dataflow-oriented Padding scheme, higher performance improvement can be achieved for layers with smaller feature maps.
% Our Dataflow-oriented Padding scheme can effectively reduce the feature map buffer time, especially for layers with small feature maps.
For an individual layer, the accelerating efficiency of our scheme is positively correlated with the proportion of padding data in the input feature maps.
Taking the content in Fig.~\ref{fig:padding} as an example for quantitative analysis, 
With uniform input dataflow, 
the direct padding scheme requires approximately $(F+2)(F+1) \times Speed_{write}$ cycles to cover a complete FM. 
In contrast, 
the time consumed by our scheme is $F^2 \times Speed_{write}$.
Accordingly,
The acceleration radio, $Radio_{acc}$, can be evaluated using the following equation:
\begin{align}\label{equ:padding radio}
    Radio_{acc} & = \frac{(F+2)(F+1) \times Speed_{write}}{F^2 \times Speed_{write}} \notag \\
    & = 1 + \frac{3}{F} + \frac{2}{F^2}
\end{align}
% where the acceleration ratio increases as the decrease of FM size.
Compared with the original scheme, an up to $1.47\times$ bandwidth enhancement for DWC layers with F=7 can be achieved in MobileNetV2 acceleration.

==> chapters/tmp/table.tex <==
\begin{table}[]
\caption{}
\label{tab:my-table}
\resizebox{\linewidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|}
\hline
                                                               & \scriptsize MACs & \scriptsize GOPS   & \begin{tabular}[c]{@{}c@{}}\scriptsize SRAM \\ \scriptsize (MB)\end{tabular} & \begin{tabular}[c]{@{}c@{}}\scriptsize DRAM Traffic\\ \scriptsize  (MB/frame)\end{tabular} & \begin{tabular}[c]{@{}c@{}}\scriptsize Latency \\ \scriptsize (ms)\end{tabular} \\ \hline
\scriptsize MobileNetV2                                                    & 1567 & 591.46 & 1.45                                                     & 2.81                                                                          & 10.63                                                   \\ \hline
\scriptsize MobileNetV2 (ZC706)  & 1569 & 588.86 & 2.00                                                     & 2.05                                                                          & 5.46                                                    \\ \hline
\scriptsize ShuffleNetV2                                                   & 1604 & 606.80 & 0.92                                                     & 1.96                                                                          & 4.74                                                    \\ \hline
\scriptsize ShuffleNetV2 (ZC706) & 1612 & 616.86 & 1.43                                                     & 0.98                                                                          & 1.33                                                    \\ \hline
\end{tabular}
}
\end{table}
